Fast hashing with Strong Concentration Bounds

Previous work on tabulation hashing by Patrascu and Thorup from STOC'11 on simple tabulation and from SODA'13 on twisted tabulation offered Chernoff-style concentration bounds on hash based sums, e.g., the number of balls/keys hashing to a given bin, but under some quite severe restrictions on the expected values of these sums. The basic idea in tabulation hashing is to view a key as consisting of $c=O(1)$ characters, e.g., a 64-bit key as $c=8$ characters of 8-bits. The character domain $\Sigma$ should be small enough that character tables of size $|\Sigma|$ fit in fast cache. The schemes then use $O(1)$ tables of this size, so the space of tabulation hashing is $O(|\Sigma|)$. However, the concentration bounds by Patrascu and Thorup only apply if the expected sums are $\ll |\Sigma|$. To see the problem, consider the very simple case where we use tabulation hashing to throw $n$ balls into $m$ bins and want to analyse the number of balls in a given bin. With their concentration bounds, we are fine if $n=m$, for then the expected value is $1$. However, if $m=2$, as when tossing $n$ unbiased coins, the expected value $n/2$ is $\gg |\Sigma|$ for large data sets, e.g., data sets that do not fit in fast cache. To handle expectations that go beyond the limits of our small space, we need a much more advanced analysis of simple tabulation, plus a new tabulation technique that we call \emph{tabulation-permutation} hashing which is at most twice as slow as simple tabulation. No other hashing scheme of comparable speed offers similar Chernoff-style concentration bounds.

==> sections/intervals.tex <==
\section{Intervals by Tabulation-1Permutation Hashing}\label{sec:intervals}
\newcommand\cD{{\mathcal D}}

We will now present a special variant of Tabulation-Permutation hashing, called
\emph{tabulation-1permutation hashing} that
is particularly tuned for hashing into intervals. At the end of this
section, we will apply this to the situation where we want to hash
keys to a number of bins that is not a power of two.

The simple idea for an efficient solution is that we only have to
permute the most significant character.

More precisely, we have a simple tabulation hash function $h\colon
\Sigma^c\to \Sigma^d$ and a single random permutation $\tau\in
S_{\Sigma}$. Then $g\colon \Sigma^c\to \Sigma^d$ is defined as
follows. To compute $g(x)$, we first set $y=(y_1, \dots, y_d)=h(x)$,
and then we return $g(x)=(\tau(y_1),y_2, \dots, y_d)$. Here we assume
that the first coordinate is the most significant in the sense that
$(y_1, \dots, y_d)$ represents the number
$\sum_{i\in[d]}|\Sigma|^{d-i}y_i$.

The advantage of tabulation-1permutation hashing is that it only uses
$c+1$ lookups regardless of $d$. Let $2^\ell=|\Sigma|^d$. We claim
that if we have $n$ balls, then for any $i<j<r$, the number of balls
hashing to the interval $[i,j)$ is tightly concentratated as in
Theorem \ref{thm:intro-tab-perm} with the additive error probability
$O(1/u^\gamma)$ where $u=|\Sigma|^c$ and $\gamma$ is an arbitrary
constant.

Let us first consider the case of a dyadic interval where $j-i=2^b$
and $i$ is a multiple of $2^b$. A key $x\in [u]$ hashes to $[i,j)$ if
and only if $g(x)$ argrees on $i$ in the first and most significant
 $\ell'=\ell-b$ bits. Now, if $2^{\ell'}\leq|\Sigma|$, then we
are only using the permuted character of $g(x)$ and then we can
apply Theorem \ref{thm:intro-tab-perm} directly to the number of
balls landing in $[i,j)$. On the other hand, if $2^{\ell'}>|\Sigma|$,
let $i=(i_1,\ldots,i_d)$, then $h(x)$ lands in $[i,j)$ if and only
if $h(x)$ argees with $(\tau^{-1}(i_1),\ldots,i_d)$ on the first
$\ell'$ bits. This is equivalent to studying the first $\ell'$
bits of $h(x)$, asking if it lands in one out of $m'=2^{\ell'}$
bins. Thus we can apply  \Cref{thm:intro-simple-tab} with $\gamma'=2c\gamma$, 
getting an addivitive error probability of $O(n/m^{\gamma'})=O(1/u^\gamma)$.

We now consider an arbitrary interval $[i,j)$. Let $k=\lfloor\log_2
(j-i)\rfloor$.  We note that $[i,j)$ can be partitioned into dyadic
intervals so that we for $h=0,\ldots,k$ have at most $2$ intervals
of size $2^h$. If we want error probabilites for a deviation of
$O(\delta)$, we do as follows.  For an intervals of size $2^h$,
the expected number of balls is $\mu_h=2^{h-\ell}$.  For each of
the at most two such intervals, we essentially want to get $(1\pm
\delta_h)\mu_h$ balls where $\delta_h=(3/2)^h\delta$. However,
pick $h_0$ as the largest number such that
$\delta_{h_0}=(3/2)^{h_0}\geq 1$. By including extra dyadic
interval of size $2^{h_0}$ on each side, we get to cover $[i,j)$
with dyadic intervals: at most $4$ of size $2^{h_0}$ and at most
$2$ of size $2^h$ for $h=h_0+1,\ldots h_k$. The total deviation
we accept is $2(1+\delta_{h_0}\mu_{h_0}+\sum_{h=h_0}^k
\delta_h\mu_h=O(\delta\mu)$, and even if we use a union bound over
the $O(k)$ involved intervals, the error probability is no worse than
in Theorem \ref{thm:intro-tab-perm}. 

All the results hold even if balls have weights in $[0,1]$ and we
condition on the hash value $r=g(q)$ of a specific query balls.

In fact, just based on the error probability bounds of dyadic intervals,
\cite{patrascu12charhash} have shown that we get deviation bounds
for the number/weight of balls ending in an interval of length at
least $L$ containing a given point $p$ which may be a function of
the hash of the query ball (they need this result for their analysis of linear probing). Applying their reduction to our
result with tabulation-1permutation hashing, which has no
limit on the expectation, we get
\begin{theorem}\label{thm:intervals}
  Consider hashing a set of 
  keys of total weight $n$ into $\{0,...,2^\ell-1\}$ 
  using tabulation-1permutation hashing. 
  Define the fill $\alpha=n/m$.  Let $p$ be any point which
  may or may not be a function of the hash value of specific query key
  not in the set. Let $\cD_{\ell,\delta,p}$ be the event that there
  exists an interval $I$ containing $p$ and of length at least $\ell$
  such that the weight $X_I$ of keys
  $X_I$ in $I$ deviates at least $\delta$ from the mean, that is,
  $|X_I-\alpha|I||\geq \delta\alpha|I|$.  Then for any constant $\gamma$.
\begin{equation}\label{eq:intervals}
\Pr[\cD_{\ell,\delta,p}]\leq \left\{\begin{array}{ll}
2e^{-\Omega(\alpha\ell\delta^2)} + (\ell/m)^{\gamma}&\mbox{if }\delta\leq 1\\
(1+\delta)^{-\Omega((1+\delta)\alpha\ell)} + (\ell/m)^{\gamma}&\mbox{if }\delta=\Omega(1)
\end{array}\right.
\end{equation}
\end{theorem}
We note that the above probability bounds are assymptotically
equivalent to those in Theorem \ref{thm:intro-tab-perm}.

\paragraph{Hashing into an arbitrary number of bins}
We now consider the case where we want to map keys of total weight $n$
to $m$ bins. If $m$ is a power of two, we already saw the most efficient
implementation in the intro. However, if $m$ is not a power of two,
we can use tabulation-1permutation hashing into $\ell$ bits where $2^\ell\gg m$.

With $2^b=|\Sigma|$ and $\texttt{>\/>}$ denoting right-shift, we define
$h^m(x)=(m\,h(x))\,\texttt{>\/>} \,(db)$ to get the most efficient and even
distribution of the keys into the $m$ bins. Now each bin corresponds
to an interval of $[2^\ell]$ of size $2^\ell/m$ rounded up or down.
The weight of the balls landing in the interval is sharply
concentrated as by Theorem \ref{thm:intervals}. The relative error due
to rounding is $m/2^{\ell}$, and thanks to tabulation-1permutation, we
use $c+1$ lookups no matter how large $\ell$ is. The only extra cost
is that we need to read and XOR longer entries.









==> sections/streaming.tex <==
\section{Fast Streaming Algorithms using Hashing with 
Strong Concentration}\label{sec:streaming}
We will illustrate the power of our new hashing schemes with
strong concentration bounds in the context of some classic algorithms for
counting distinct elements and for estimating set similarity. In the two applications below, it suffices to use tabulation-1permutation to obtain strong guarantees.

\subsection{Counting distinct elements in a data strem}
We consider a sequence of keys $x_1,\ldots,x_s \in [u]$ where each
element may appear multiple times. Using only little space, we wish to
estimate the number $n$ of distinct keys. We are given parameters
$\eps$ and $\delta$, and goal is to create an estimator, $\hat n$, such that $(1-\eps) n \leq \hat n \leq  (1+\eps) n$ with probability at least $1-\delta$.

Following the classic approach of Bar-Yossef et al.~\cite{BJKST02}, we
use a hash function $h:U\to (0,1]$ which we assume to be collision free
  over $U$. For some $k>1$, we maintain the $k$ smallest distinct hash
  values of the stream. We assume for simplicity that $k\leq n$. The space required is thus $O(k)$, so we want $k$ to be small.  Let $x_{(k)}$ be the key having the $k$'th smallest hash value under $h$ and let $h_{(k)}=h(x_{(k)})$. As in~\cite{BJKST02}, we use $\hat n=k/h_{(k)}$ as an estimator for
  $n$ (we note that \cite{BJKST02} suggests several other estimator,
  but the points we will make below with our new Tabulation-1Permutation hashing 
  apply to all of them).

The point in using a hash function $h$ is that all occurrences of a given
key $x$ in the stream get the same hash value, so if
$S$ is the set of distinct keys, $h_{(k)}$ is
just the $k$ smallest hash value from $S$. In particular, $\hat n$ depends only on $S$, not on the frequencies of the elements of the stream.
Assuming no
collisions, we will often identify the elements with
the hash values, so $x_i$ is smaller than $x_j$ if
$h(x_i)\leq h(x_j)$.

We would like $1/h_{(k)}$ to be concentrated
around $n/k$. For any probability $p\in[0,1]$, let
$X^{<p}$ denote the number of elements from $S$ that hash below $p$.
Let $p_-=k/((1+\eps)n)$ and $p_+=k/((1-\eps)n)$. Note that both $p_-$ and
$p_+$ are independent of the random hash function $h$. Now 
\begin{align*}
1/h_{(k)}&\leq (1-\eps)n/k\iff X^{<p_+}< k=(1-\eps)\E{X^{<p_+}}\\
1/h_{(k)}&> (1+\eps)n/k\iff X^{<p_-}\geq k=(1+\eps)\E{X^{<p_-}},
\end{align*}
and these observations form a good starting point for applying probabilistic tail bounds as we now describe.
\paragraph{Using 2-independence and independent repetitions}
Bar-Yossef et al. \cite{BJKST02} suggested using 
a 2-indendent hash function. Then, for any $p$, we have 
$\Var{X^{<p}}\leq \E{X^{<p}}$, so by Chebyshev's inequality,
 
\begin{align*}
\PR{1/h_{(k)}\leq (1-\eps)n/k}&<(1-\eps)/(k\eps^2)\\
\PR{1/h_{(k)}>(1+\eps)n/k}&\leq(1+\eps)/(k\eps^2).
\end{align*}
Assuming $\eps\leq 1$, we thus get that
\[\PR{|\hat n -n|> \eps n}=\PR{\left|1/h_{(k)}-n/k\right| > \eps n/k}\leq 3/(k\eps^2).\]
To get the a desired error probability $\delta$, we could now set
$k=3/(\delta\eps^2)$, but if $\delta$ is small, e.g. $\delta=1/u$, $k$ becomes way too large. As in~\cite{BJKST02} we instead start by aiming for a constant error probability, $\delta_0$, say $\delta_0=1/4$. For this value of $\delta_0$, it suffices to set $k_0=12/\eps^2$. We now run $r$ (to be
determined) independent experiments with this value of $k_0$, obtaining independent estimators for $n$, $\hat n_1,\ldots,\hat n_r$. Finally, as our final estimator, $\hat n$, we return the median of $\hat n_1,\dots,\hat n_r$. Now for each $1\leq i \leq r$, $\Pr[|\hat n_i-n|> \eps n]\leq 1/4$ and these events are independent. If $|\hat n-n|\geq \eps n$, then $|\hat n_i-n|\geq \eps n$ for at least half of the $1\leq i \leq r$. By the standard Chernoff bound~\req{eq:classic-chernoff+}, this probability can be bounded by 
\[\PR{|\hat n -n|> \eps n}
\leq \exp(-(r/4)/3)=\exp(-r/12).\] 
Setting $r=12\ln(1/\delta)$, we get
the desired error probability $1/\delta$. The total number of hash
values stored is
$k_0r=(12/\eps^2)(12\ln(\delta))=144\ln(1/\delta)/\eps^2$.



\paragraph{A better world with fully random hashing}
Suppose instead that $h:[u]\to (0,1]$ is a fully random hash function.
In this case, the standard Chernoff bounds \req{eq:classic-chernoff+} and
\req{eq:classic-chernoff-} with $\eps\leq 1$ yield
\begin{align*}
\PR{1/h_{(k)}\leq (1-\eps)n/k}&<\exp(-(k/(1-\eps))\eps^2/2))\\
\PR{1/h_{(k)}>(1+\eps)n/k}&\leq\exp(-(k/(1+\eps))\eps^2/3)).
\end{align*}
Hence
\begin{equation}\label{eq:stream-Chernoff}
\PR{|\hat n -n|> \eps n}=\PR{|1/h_{(k)}-n/k|\geq \eps n/k}
\leq 2\exp(-k\eps^2/6).
\end{equation}
Thus, to get error probability $\delta$, we just use $k=6\ln(2/\delta)/\eps^2$.
There are several reasons why this is much better than the above approach
using 2-independence and independent repetitions.
\begin{itemize}
\item It avoids the independent repetitions, so instead of
applying $r=\Theta(\log(1/\delta))$ hash functions to each key we just need one. We thus save a factor of $\Theta(\log(1/\delta))$ in speed. 
\item Overall we store fewer hash values: 
$k=6\ln(2/\delta)/\eps^2$
instead of $144\ln(1/\delta)/\eps^2$.
\item With independent repetitions, we are tuning the algorithm depending on $\eps$ and
$\delta$, whereas with a fully-random hash function, we get the
concentration from \req{eq:stream-Chernoff} for every $\eps\leq 1$.
\end{itemize}
The only caveat is that fully-random hash functions cannot be implemented.
\paragraph{Using Tabulation-1Permutation hashing}
We now discuss the guarantees obtained by implementing the second scheme above with Tabulation-1Permutation hashing.
Ignoring small rounding errors, we think of the output bit strings
as uniform in $(0,1]$. By 
Theorem~\ref{thm:intro-tab-1perm}, and using that for any $p$, $\Var{X^{<p}}\leq \E{X^{<p}}$,
\begin{align*}
\PR{1/h_{(k)}\leq (1-\eps)n/k}&=2\exp(-\Omega(k/(1-\eps))\eps^2))+1/u^\gamma\\
\PR{1/h_{(k)}>(1+\eps)n/k}&=2\exp(-\Omega(k/(1+\eps))\eps^2/3))+1/u^\gamma.
\end{align*}
Assuming $\eps\leq 1$, it follows that
\begin{equation}\label{eq:stream-perm1}
\PR{|\hat n-n| \geq \eps n}=\PR{|1/h_{(k)}-n/k| \geq \eps n/k}
\leq 2\exp(-\Omega(k\eps^2)) +1/u^\gamma.
\end{equation}
To obtain the error probability $\delta$, 
we again need to store $k=O(\log(1/\delta)/\eps^2)$ hash values.
Within a constant factor this means that we use the same total number
using 2-independence and independent repetitions, and we still
retain the following advantages from the fully random case.
\begin{itemize}
\item With no independent repetitions we avoid
applying $r=\Theta(\log(1/\delta))$ hash functions to each key,
so we basically save a factor $\Theta(\log(1/\delta))$ in speed. 
\item With independent repetitions, we only address a given $\eps\leq 1$ and
$\delta$, while with a fully-random hash function we get the
concentration from \req{eq:stream-Chernoff} for every $\eps\leq 1$.
\end{itemize}
We note that it is crucial for this application that we can
handle a fairly large expected value $\mu$ --- for the lower bound, $\mu=k/(1-\eps)$. Even in the
fully random case we used $k=6\ln(2/\delta)/\eps^2$,
so with, say, $\delta=1/2^{30}$ and $\eps=1\%$, we
get $\mu\geq k> 2^{20}$. This would be serious problem with, e.g,
the twisted tabulation from \cite{PT13:twist} which requires
$\mu<|\Sigma|^{1-\Omega(1)}$. Indeed, for the character tables to fit in fast cache, we have to choose $|\Sigma|$ rather small, e.g. $|\Sigma|=2^8$.
\paragraph{Implementation and alternatives}
We briefly discuss how to maintain the $k$ smallest elements/hash values.  The
most obvious method is using a priority queue, but this takes
$O(\log k)$ time per element, dominating the cost of evaluating the hash
function. However, we can get down to constant time per element if
have a buffer for $k$. When the buffer gets full, we find the median in linear time with (randomized) selection and discard the bigger elements. This is standard to deamortize if needed. 

A different, and more efficient, sketch from~\cite{BJKST02} identifies the smallest $b$ such that the number
$X^{<1/2^b}$ of keys hashing below $1/2^b$ is at most $k$. For the
online processing of the stream, this means that we increment $b$
whenever $X^{<1/2^b}>k$. At the end, we return $2^b X^{<1/2^b}$.
The analysis of this alternative sketch is similar to the one
above, and we get the same advantage of avoiding independent
repetitions using the strong concentration guaranteed when implementing the hashing with tabulation-1permutation.
  
Another issue is that we need to maintain some kind of hash table over
the stored elements to check whether a new element is already stored. One
nice advantage of using tabulation-1permutation hashing is that we can
use the least significant bits of the original hash function to
index the hash table. The basic point is that
if we generate $\ell$-bit hash values with simple tabulation, then these $\ell$ bits
are completely independent. The cost in time with a larger $\ell$
is very small because we do exactly the same number of lookups.
The difference is that the entries are larger.
With $\ell=\ell_0+\ell_1$, we can
use the first $\ell_0$ bits as part of the tabulation-1permutation hashing (which then proceeds by permuting the first character).
The last $\ell_1$ bits can be used to index
the hash table over the keys stored. 

\paragraph{Space}
There has been a lot of work on how to represent a sketch for distinct
elements using as few bits as possible (see, e.g.,
\cite{BJKST02,Bla18:stream,JW13:stream-lb,KNW10:stream}), and now we know that
$O(\log(1/\delta)/\eps^2+\log n)$ bits is best possible
\cite{JW13:stream-lb,KNW10:stream}. However, all these approaches use
the idea of computing $O(\log(1/\delta)$ different
hash functions (even though they may not be completely independent).

Our work is orthogonal in its focus on time. Our hash functions alone
use space $(c+1)u^{1/c}$, $c=O(1)$, where $u$ is the size of the
universe, which in theory is much larger, but plugging in real numbers
such as $c=8$ for $u=2^{64}$, we can get fast hashing with strong
concentration bounds, and then we avoid the multiplicative factor
$O(\log(1/\delta))$. 



\subsection{Set similarity} 
\newcommand\MIN{\textnormal{MIN}}
We now consider Broder's~\cite{Broder97onthe}
original algorithm for set similarity. As above,
it uses a hash function $h:[u]\to[0,1]$ which we
assume to be collision free. The bottom-$k$ sample $\MIN_k(S)$ of a set 
$S\subseteq [u]$ consists of the $k$ elements with the smallest
hash values. If $h$ is fully random then $\MIN_k(S)$ is a uniformly
random subset of $k$ distinct elements from $\MIN_k(S)$. We assume
here that $k\leq n=|S|$.
With $\MIN_k(S)$, we can
estimate the frequency $f=|T|/|S|$ of any subset $T\subseteq S$ as 
$|\MIN_k(S)\cap T|/k$. 

Broder's main application is the estimation of the Jaccard
similarity $f=|A\cap B|/|A\cup B|$ between sets $A$ and $B$. Given the
bottom-$k$ samples from $A$ and $B$, we may construct the bottom-$k$ sample of
their union as $\MIN_k(A\cup B)=\MIN_k(\MIN_k(A)\cup \MIN_k(B))$, and then the
similarity is estimated as $|\MIN_k(A\cup B)\cap \MIN_k(A)\cap \MIN_k(B)|/k$.


We note again the crucial importance of having a common hash
function $h$. In a distributed settings, samples $\MIN_k(A)$ and $\MIN_k(B)$
can be generated by different entities. As long as
they agree on $h$, they only need to communicate the samples to estimate
the Jaccard similarity of $A$ and $B$. 

For the hash function $h$, Broder \cite{Broder97onthe} first considers
fully random hashing, and then he sketches some more realistic
alternatives. Thorup \cite{thorup13bottomk} showed that even if we
just use 2-independence, we get the same expected error as with fully
random hashing. Here we want strong concentration using a single
tabulation-1permutation hash function. Our analysis follows the simple
union-bound approach from \cite{thorup13bottomk}.

Concerning the sharing of a tabulation-1permutation hash function $h$,
recall that, in order to obtain our strong concentration bounds, it suffices to fill the character tables using a $O(\log u)$-independent pseudo-random number generator in the preprocessing step. As the output characters are bit string of length $O(\log u)$, this requires a $O(\log^2 u)$-bit seed, and it is only this seed that different processors need to
communicate and agree on.



For the analysis, it is simpler to study the case where
we are sampling from a set $S$ and want to estimate the
frequency $f=|T|/|S|$ of a subset $T\subseteq S$. Let
$h_{(k)}$ be the $k$th smallest hash value from $S$ as
in the above algorithm for estimating distinct elements.
For any $p$ let $Y^{\leq p}$ be the number of elements
from $T$ with hash value at most $p$. Then
$|T\cap \MIN_k(S)|=Y^{\leq h_{(k)}}$ which is our estimator for $fk$.

\begin{theorem}
For $\eps\leq 1$ and any $\gamma=O(1)$
\begin{equation}\label{eq:sim-small-eps}
\PR{|Y^{\leq h_{(k)}}-fk|>\eps fk}=2\exp(-\Omega(fk\eps^2))+1/u^{\gamma}.
\end{equation}
For $\eps\geq 1$ and any $\gamma=O(1)$
\begin{align}\label{eq:sim-large-eps}
\PR{Y^{\leq h_{(k)}}>(1+\eps)fk}=2\exp(-\Omega(fk\,\cC(\eps))+2\exp(-\Omega(k))+1/u^{\gamma}.
\end{align}
\end{theorem}
\begin{proof}
Let $n=|S|$. Using tabulation-1permutation hashing, we already saw
in \req{eq:stream-Chernoff} that for any $\eps_S\leq 1$ and $\gamma=O(1)$,
\(P_S=\PR{|1/h_{(k)}-n/k|\geq \eps_S n/k}\leq 2\exp(-\Omega(k\eps_S^2)) +
1/u^\gamma.
\) 
Thus, with $p_-=k/((1+\eps_S)n)$ and $p_+=k/((1-\eps_S)n)$,
we have $h_{(k)}\in [p_-,\,p_+]$ with probability $1-P_S$, and in
that case, $Y^{\leq p_-}\leq Y^{\leq h_{(k)}}\leq Y^{\leq p_+}$. 

Let $\mu^-=\E{Y^{\leq p_-}}=fk/(1+\eps_S)\geq fk/2$.  By 
Theorem \ref{thm:intro-tab-1perm}, and using that the expectation dominates the variance, for any $\eps_T\leq 1$, we get that 
\[P^-_{T}=\PR{Y^{\leq p_-}\leq (1-\eps_T)\mu_-}\leq 2\exp(-\Omega(\mu_-\eps_T^2))+1/u^\gamma
= 2\exp(-\Omega(fk\eps_T^2))+1/u^\gamma.\]
Thus
\[\PR{Y^{\leq h_{(k)}}\leq \frac{1-\eps_T}{1+\eps_S}fk}\leq P^-_T+P_S.\]
Likewise, with $\mu^+=\E{Y^{\leq p_+}}=fk/(1-\eps_S)$, for any $\eps_T$,
we get that
\begin{align*}
P^+_T=\PR{Y^{\leq p_+}\geq (1+\eps_T)\mu_+}
\leq 2\exp(-\Omega(\mu_+\eps_T^2))+1/u^\gamma 
= 2\exp(-\Omega(fk\eps_T^2))+1/u^\gamma,
\end{align*}
and
\begin{align*}
\PR{Y^{\leq h_{(k)}}\geq \frac{1+\eps_T}{1-\eps_S}fk}\leq P^+_T+P_S.
\end{align*}
To prove the theorem for $\eps\leq 1$, we set $\eps_S=\eps_T=\eps/3$. Then
$\frac{1+\eps_T}{1-\eps_S}\leq 1+\eps$ and 
$\frac{1-\eps_T}{1+\eps_S}\geq 1-\eps$. Therefore
\[\PR{|Y^{\leq h_{(k)}}-fk|\geq \eps fk}\leq P^-_T+P^+_T+2P_S\leq
8\exp(-\Omega(fk\eps_T^2))+4/u^\gamma= 2\exp(-\Omega(fk\eps_T^2))+1/u^{\gamma'}\]
where $\gamma'=\gamma-1/\log_4 u$. This completes the proof
of \req{eq:sim-small-eps}.

Now, for $\eps> 1$, we fix $\eps_S=1/3$ while $\eps_T=\eps/3$. We
are now only concerned with too large estimates. Then $\frac{1+\eps_T}{1-\eps_S}\leq 1+\eps$. This time, we apply Theorem \ref{thm:intro-tab-1perm}
with the more general formula that is valid for all $\eps_T$,
yielding
\[P^+_{T}=\PR{Y^{\leq p_+}\geq (1+\eps_T)\mu_+} \leq 
2\exp(-\Omega(fk\,\cC(\eps_T))+1/u^\gamma.\]
Now we have 
\[\PR{Y^{\leq h_{(k)}}\geq (1+\eps)fk}
\leq\PR{Y^{\leq h_{(k)}}\geq \frac{1+\eps_T}{1-\eps_S}fk}
\leq P^++P_S\leq 2\exp(-\Omega(k/4)) +
2\exp(-\Omega(fk\,\cC(\eps_T))+1/u^{\gamma'}.\]
By~\Cref{lem:Benn-func-consts}, $\cC( \eps_T)=\Theta(\cC(\eps))$ and the proof of \req{eq:sim-small-eps} is complete.
\end{proof}
As for the problem of counting distinct elements in a stream, in the online setting we may again modify the algorithm above to obtain a more efficient sketch. Assuming that the elements from $S$ appear in a stream, we again identify the smallest $b$ such that, the number of keys from $S$ hashing below $1/2^b$, $X^{\leq 1/2^b}$, is at most $k$. We increment $b$ by one whenever $X^{\leq 1/2^b}>k$ and in the end we return $Y^{\leq 1/2^b}/X^{\leq 1/2^b}$ as an estimator for $f$. The analysis of this modified algorithm is similar to the analysis provided above.



==> sections/technical_overview.tex <==
\section{Techniques}
We apply a string of new techniques and ideas to arrive at the two main theorems of the paper.
The exposition is subdivided into three parts, each yielding theorems of independent interest. Combining these yields \cref{thm:intro-simple-tab} and \cref{thm:intro-tab-perm}, but in fact in both cases imply even stronger statements. Below we present the main theorem of each section and show how they imply \cref{thm:intro-simple-tab} and \cref{thm:intro-tab-perm}. This is followed by a technical description of each section and of how each of the main theorems come about.

\paragraph{Simple Tabulation}
The first part of this paper (\Cref{sec:simple}) presents a much tighter analysis of simple tabulation hashing,
proving concentration bounds for throwing weighted balls into bins.
This includes an analysis of the case of general value functions with restricted support, not
just one as in Theorem 1.
Our main theorem of \Cref{sec:simple} is the following.
\begin{theorem}\label{thm:simpleConcentration}
    Let $h\colon \Sigma^c \to [m]$ be a simple tabulation hash function and
    $S \subseteq \Sigma^c$ be a set of keys. Let $w\colon \Sigma^c \times [m] \to [-1, 1]$ be
    a value function such that the set
    $Q = \setbuilder{i \in [m]}{\exists x \in \Sigma^c : w(x, i) \neq 0}$ satisfies  $\abs{Q} \le m^{\eps}$,
    where $\eps < \frac{1}{4}$ is a constant.
    Define the random variable
    \[
        W = \sum_{x \in S} \sum_{k \in Q} w(x, k)\left([h(x) =  k] -\frac{1}{m}\right) \; ,
    \]
    and $\sigma^2 = \Var{W} $.
    For any constant $\gamma \geq 1$ the following bounds hold:
    \begin{align}
        \PR{\abs{W} \ge C_{\gamma, c} t}
            \le  2\exp\left(-\sigma^2 \C\left(\frac{t}{\sigma^2}\right)\right)
                + O_{\gamma, \eps, c}\left(\abs{S} m^{-\gamma}\right) \; , \label{eq:Chernoff}
       \end{align}
       \begin{align}
       \PR{\sum_{j \in [m]}\left( \sum_{x \in S}\sum_{k \in Q}
            w(x, k)\left([h(x) = j \oplus k] -\frac{1}{m}\right)
        \right)^2 > D_{\gamma, c} \left(\sum_{x \in S}\sum_{k \in Q} w(x, k)^2 \right)}
           = O_{\gamma, \eps, c}(|S|m^{-\gamma}) \; , \label{eq:squares}
    \end{align}
    for some large enough constants $C_{\gamma, c}$,$D_{\gamma, c}$. Here $\mathcal{C}: \R_{\geq 0} \to \R_{\geq 0}$ maps $x\mapsto (x+1)\log (x+1)-x$. This result holds even when the value function depends on the hash of a query key $q\in [u]\setminus S$ (with $C_{\gamma,c}$ and $D_{\gamma, c}$ slightly larger).

% Let $h\colon \Sigma^c\to [m]$ be a simple tabulation hash function and for every $x\in \Sigma^c$
% let $w_x\in [0, 1]$ be the weight of $x$. Let $S\subset \Sigma^c$ be a set of keys with $\norm{S}_\infty=1$
% and $y\in [m]$ a bin. Define the stochastic variable
%     $$
%     W=\sum_{x \in S} w_x \cdot\left([h(x)=y]- \frac{1}{m} \right),
%     $$
%     and $\sigma^2=\Var{W}= \norm{S}_2^2\left(m^{-1}-m^{-2} \right)$. For any $\delta \geq 0$ and $\gamma=O(1)$,
%     $$
%     \Pr[|W|\geq \delta \sigma^2] \leq 2e^{-\Omega_{c,\gamma}(h(\delta) \sigma^2)}+O_{c,\gamma}(nm^{-\gamma}).
%     $$
\end{theorem}
The theorem can be seen as a tight analysis of the use of simple tabulation hashing towards concentration bounds, thus completing a part of the line of research~\cite{DKRT15:k-part,patrascu12charhash,PT13:twist,Tho13:simple-simple} started by P{\v a}tra{\c s}cu and Thorup in~\cite{patrascu12charhash} on concentration with tabulation hashing.
~\cref{eq:squares} of the theorem is an important technical tool. It is proved first and then used in the proof of~\cref{eq:Chernoff}. Later it is then applied in the analysis of the performance of tabulation-permutation hashing.

Let us briefly argue that~\Cref{thm:simpleConcentration} implies~\Cref{thm:intro-simple-tab}. Assume that we are in the setting of~\Cref{{thm:intro-simple-tab}} and let $w:\Sigma^c \times [m] \to [0,1]$ be defined by
$$
w(x,k)=\begin{cases}
w_x, & \text{if } k=t \text{ and } x\in S\\
0, & \text{otherwise}
\end{cases}
$$
Applying~\cref{eq:Chernoff} of~\Cref{thm:simpleConcentration} with $Q=\{t\}$ and $W=V-\mu=\sum_{x \in S} \sum_{k \in Q} w(x, k)\left([h(x) =  k] -\frac{1}{m}\right)$ we find that
$$
\Pr[V\geq (1+\delta )\mu] \le 2\exp\left(-\sigma^2 \C\left(\frac{\delta \mu}{C_{\gamma,c}\sigma^2}\right)\right)
                + O_{\gamma, c}\left(n m^{-\gamma}\right)
$$
Now $\sigma^2=\sum_{x\in S}w_x^2 (1/m-1/m^2)\leq \mu$ and it is an easy exercise (and the content of the upcoming~\Cref{lem:Benn-func-var-and-max}) to show that the bound above only gets worse if $\sigma^2$ is replaced by a larger number. One can moreover show that $\mathcal{C}(\alpha x)=\Theta(\mathcal{C}(x))$ for $\alpha=\Theta(1)$ -- this is the content of the upcoming~\Cref{lem:Benn-func-consts}). Combining these two observations it follows that
$$
\Pr[V\geq (1+\delta )\mu] \le 2\exp\left(-\Omega (\mu \C(\delta)\right))
                + O_{\gamma, c}\left(n m^{-\gamma}\right) =2 \left(\frac{e^\delta}{(1+\delta)^{1+\delta}} \right)^{\Omega (\mu)}+O_{\gamma, c}\left(n m^{-\gamma}\right).
$$
The bound on $\Pr[V\leq (1-\delta )\mu]$ is proved similarly, and when $t$ is a function of the hash of a query $q\in U \setminus S$ we proceed as above using the corresponding part of~\Cref{thm:simpleConcentration}.

\paragraph{Permutation}
The second part of the paper (\Cref{sec:valuefunctions}) proves that given a hash
function with concentration bounds like~\eqref{eq:Chernoff} and~\eqref{eq:squares}
in~\Cref{thm:simpleConcentration}, composing with a uniformly random permutation
of the entire codomain yields a hash function giving Chernoff-type concentration
for general value functions. The main theorem of \Cref{sec:valuefunctions} is the following.
%The second part of the paper proves that composing a simple tabulation hash function with a uniformly random permutation of the entire codomain yields a hash function that can handle any general value function. The main theorem is the following.
\begin{theorem}\label{thm:valuefunctions}
    For a set $S$, an integer $m \ge 2$ and a positive number $\eps \in (0, 1]$,
    let $h \colon S \to [m]$ be a 2-independent hash function satisfying the following.
    For every value function $w \colon S \times [m] \to [-1, 1]$ such that the set
    $Q = \setbuilder{i \in [m]}{\exists x \in S : w(x, i) \neq 0}$ satisfies $\abs{Q} \le m^\eps$,
    and every $\gamma >0$,~\cref{eq:Chernoff,eq:squares} of~\Cref{thm:simpleConcentration} hold.
   % \begin{align}
     %   \PR{\abs{ \sum_{x \in S} \sum_{i \in Q} w(x, i) \left( [h(x) = i] - \frac{1}{m} \right) } \ge C \cdot t}
    %       &\le 2 \exp\left(-\sigma^2 \C\left(\frac{t}{\sigma^2}\right)\right) + O(|S|m^{-\gamma}) \; ,  \\
     %   \PR{\sum_{j \in [m]} \left( \sum_{x \in S} w(x, k) \left( [h(x) = k \oplus j] - \frac{1}{m} \right) \right)^2 \ge D \cdot \sum_{x \in S} w(x, k)^2}
    %        &= O(|S|m^{-\gamma}) \; ,
  %  \end{align}
   % where $k \in Q$, $\sigma^2 = \Var{\sum_{x \in S} \sum_{i \in Q} w(x, i) \left( [h(x) = i] - \frac{1}{m} \right)}$,
   % and $C$ and $D$ are universal constants depending on $\eps$ and $\gamma$.

    Let $w' : S \times [m] \to [-1, 1]$ be any value function,
    %with the property that $\sum_{i \in [m]} w(x, i) = 0$ for every $x \in S$,
    $\tau : [m] \to [m]$ a uniformly random permutation independent of $h$, and $\gamma>0$, then
    \begin{align*}
        \PR{\abs{ \sum_{x \in S} \sum_{i \in [m]} w'(x, i) \left( [\tau(h(x)) = i] - \frac{1}{m} \right) } \ge E \cdot t}
            \le 2 \exp\left(-\sigma^2 \mathcal{C}\left(\frac{t}{\sigma^2}\right)\right) + O(|S|m^{-\gamma}) \; ,
    \end{align*}
    where $\sigma^2 = \Var{\sum_{x \in S} \sum_{i \in [m]} w'(x, i) \left( [\tau(h(x)) = i] - \frac{1}{m} \right)}$,
    and $E$ is a universal constant depending on $\gamma$ and $\eps$. This result holds (with slightly larger constants) even when the value function depends on the hash value of a query key $q\in [u]$. The only requirement is that in that case the assumptions on $h$ must also hold under this condition.
\end{theorem}
We believe the theorem to be of independent interest. From a hash function that only performs well for value functions supported on an asymptotically small subset of the bins we can construct a hash function performing well for any value function -- simply by composing with a random permutation.~\Cref{thm:simpleConcentration} shows that simple tabulation satisfies the two conditions in the theorem above. It follows that if $m=|U|^{\Omega(1)}$, e.g., if $m=|\Sigma|$, then composing a simple tabulation hash function $h:\Sigma^c \to [m]$ with a uniformly random permutation $\tau:[m] \to [m]$ yields a hash function $\tau \circ h$ having Chernoff-style bounds for general value functions asymptotically matching those from the fully random setting up to an additive error inversely polynomial in the size of the universe.
In particular these bounds hold for tabulation-permutation hashing from $\Sigma^c$ to $\Sigma$, that is, using just a single permutation, which yields the result of~\Cref{thm:intro-tab-perm} in the case $d=1$. If we desire a range of size $m\gg |\Sigma|$ the permutation $\tau$ becomes too expensive to store. In tabulation-permutation hashing $\Sigma^c \to \Sigma^d$ we instead use $d$ permutations $\tau_1,\dots, \tau_d:\Sigma \to \Sigma$, hashing
$$
\Sigma^c \xrightarrow[]{h^{\text{simple}}} \Sigma^{d} \xrightarrow[]{(\pi_1,\dots,\pi_d)} \Sigma^d.
$$

\paragraph{Concatenation}
The third and final part of the paper (\Cref{sec:codomainext}) shows that
concatenating the hash values of two independent hash functions each with Chernoff-style
bounds for general value functions yields a new hash function with a larger codomain and
similar Chernoff-style bounds with only a constant blow up of the constants.
In particular it will follow that tabulation-permutation hashing has Chernoff-style
bounds for general value functions. The main theorem of \Cref{sec:codomainext} is the following.
\begin{theorem}\label{thm:extendingCodomain}
    Let $A$ be a finite set. Let $X=(X_a)_{a\in A}$ and $Y=(Y_a)_{a\in A}$ be pairwise independent families of random variables taking values in $B_X$ and $B_Y$, respectively, and satisfying that the distributions of $(X_a)_{a\in A}$ and $(Y_a)_{a\in A}$ are independent.
    Suppose that $D_X, D_Y\geq 1$, $K_X, K_Y>0$, and $r_X, r_Y\geq 0$ are such that for every choice of weight functions $w_X\colon A\times B_X\to [0, 1]$ and $w_Y\colon A\times B_Y\to [0, 1]$ and for every $\delta>0$,
    \begin{align}\label{PT1_introduction}
        P\left( \abs{\sum_{a\in A} w_X(a, X_a)-\mu_X} >D_X\cdot \delta\cdot \mu_X \right)&<K_X\exp\left( -\mu_X \cdot \C(\delta) \right) +r_X,\\ \label{PT2_introduction}
        P\left( \abs{\sum_{a\in A} w_Y(a, Y_a)-\mu_Y} >D_Y \cdot\delta\cdot \mu_Y \right)&<K_Y\exp\left(-\mu_Y\cdot \C(\delta)\right) + r_Y,
    \end{align}
    where $\mu_X = \E{\sum_{a\in A} w_X(a, X_a)}$ and $\mu_Y = \E{\sum_{a\in A} w_Y(a, Y_a)}$. Then for every weight function $\overline w\colon A\times B_X\times B_Y\to [0, 1] $ and every $\delta>0$,
    \begin{align*}
        P\left( \abs{\sum_{a\in A}\overline w(a, X_a, Y_a)-\mu_{XY}}>D_{XY}\cdot\delta\cdot \mu_{XY} \right)<K_{KY}\cdot \exp\left(-\mu_{XY}\cdot \C(\delta)\right)+r_{XY},
    \end{align*}
    where $\mu_{XY}=\E{\sum_{a\in A}\overline w(a, X_a, Y_a)}$, $D_{XY} = 5D_X\cdot (1+2D_Y)$, $K_{XY} = 2K_X+K_Y$, and $r_{XY}=2r_X+r_Y$.
\end{theorem}
As with~\Cref{thm:valuefunctions}, this result is of independent interest. Since it uses the input hash functions in a black box manner it functions as a general tool towards producing hash functions with Chernoff-style bounds.

We proceed to argue that~\Cref{thm:extendingCodomain,thm:simpleConcentration,thm:valuefunctions}  imply~\Cref{thm:intro-tab-perm}. Suppose that we are in the setting of~\cref{thm:intro-tab-perm}. The arguments succeeding~\Cref{thm:valuefunctions} show that in the case $d=1$ and for any value function $w$,
  \begin{align*}
        \PR{|V-\mu| \ge E \cdot t}
            \le 2 \exp\left(-\sigma^2 \mathcal{C}\left(\frac{t}{\sigma^2}\right)\right) + O(u^{-\gamma}) \; ,
    \end{align*}
for some constant $E$ depending on $\gamma$ and $c$. Applying~\Cref{thm:extendingCodomain}, $\lceil \lg d \rceil$ times, we find that even for $d\geq 1$,
  \begin{align*}
        \PR{|V-\mu| \ge E' \cdot t}
            \le 2 \exp\left(-\sigma^2 \mathcal{C}\left(\frac{t}{\sigma^2}\right)\right) + O(u^{-\gamma}) \; ,
    \end{align*}
for some constant $E'$  depending on $\gamma,c$ and $d$. At this point an argument similar to that following~\Cref{thm:simpleConcentration} completes the proof.


\subsection{Analysis of Simple Tabulation}
A large part of the technical contribution of this paper is spent on a thorough analysis of simple tabulation in~\Cref{sec:simple}. We pick up the basic approach in the analysis by P{\v a}tra{\c s}cu and Thorup \cite{patrascu12charhash} and generalize and extend it to obtain strong, general concentration bounds. The pinnacle of the section is the proof of~\Cref{thm:simpleConcentration}.


The key idea of P{\v a}tra{\c s}cu and Thorup \cite{patrascu12charhash} was to perform the analysis of the concentration in the following way. Consider a simple tabulation function $h\colon \Sigma^c\to [m]$. Define a \emph{position character} to be an element of $[c]\times \Sigma$. We can then consider a key $x=(x_1, \dots, x_c)\in \Sigma^c$ as a set containing the position characters $(1, x_1), \dots, (c, x_c)\in [c]\times \Sigma$. With this view in mind, we shall write $(i, x_i)\in x$ if $(i, x_i)$ is a position character of $x$. If $h_1,\dots,h_c: \Sigma \to [m]$ and $h:=\Sigma^c\to [m]$ is defined by $h(x) = \bigoplus_{i=1}^ch_i(x_i)$, we overload notation by letting $h(\alpha)=h_a(y)$ for a position character $\alpha=(a, y)\in [c]\times \Sigma$. For a set $S\subset[c]\times \Sigma$ of position characters we further write $h(S)=\oplus_{\alpha \in S} h(\alpha)$.
Suppose $\prec$ is an order on the set of position characters and enumerate the position characters $\alpha_1 \prec \cdots\prec\alpha_r$ according to this order. %N ow, suppose that we order the set of position characters $\{\alpha_1, \dots, \alpha_r\} = [c]\times \Sigma$ such that $\alpha_i\prec \alpha_j$ if and only if $i<j$.
For a set of keys $S\subset \Sigma^c$ and every $j\in [r]$, we can then define the \emph{group} of keys $x$ that contain the position character $\alpha_j$ and satisfy that $\alpha_j$ is the maximal position character of $x$ with respect to the ordering $\prec$,
$$G_j = \{ x\in S \mid \alpha_j\in x\subseteq \{ \alpha_1, \dots, \alpha_j \} \}.$$
We can view the process of randomly picking a simple tabulation hash function as sequentially fixing the value of $h(\alpha_j)$ for $j\in [r]$ uniformly at random in the order $\prec$.
Immediately before fixing the hash value $h(\alpha_j)$ the internal clustering of the keys of $G_j$ has been determined in the sense that $h(x \setminus \{\alpha_j\})$ has been determined for all $x\in G_j$, and after fixing the hash of $\alpha_j$ these values are each shifted by an XOR with $h(\alpha_j)$.
% When fixing the value of $h(\alpha_j)$, every key $x\in G_j$ will have its final assignment $h(x)$ fixed and the value of $h(x)$ will be independent of every key of $\bigcup_{i=1}^{j-1}G_i$. However, $h(x)$ and $h(y)$ for $x, y\in G_j$ will be very much correlated given the value of $h(\alpha_i)$ for every $i<j$.
Now, P{\v a}tra{\c s}cu and Thorup prove that the ordering $\alpha_1\prec \dots \prec \alpha_r$ can be chosen such that for each $j\in [r]$, $\abs{G_j}\leq \abs S^{1-1/c}$. This fact together with the following trick enables them to prove concentration results on the number of balls landing in a given bin $t$.
% This fact together with the following trick enables them to bound the aforementioned correlation.
The proof is inductive, viewing the situation before each step $j\in [r]$ as though the set of keys $G_j$ has already been hashed into $m$ bins by a simple tabulation function $h'\colon \Sigma^{c-1}\to [m]$. The fixing of the last position character of each key of $G_j$ then ``rotates'' the image of $G_j$ under $h'$, $h'(G_j)$, into $h(G_j)$ by the operation $h(\alpha_j)\oplus h'(G_j)$. The inductive hypothesis applied to the groups $G_j$ combined with the contribution of each group being relatively small ($|G_j|\leq |S|^{1-1/c}$) then allows them to prove concentration bounds.

We rely on this idea and framework too. However, we generalize the framework significantly, greatly extending the theory of simple tabulation hashing and obtaining tighter concentration bounds. %The first thing to mention is that we study simple tabulation hashing with value  as in~\Cref{thm:simpleConcentration}.
This makes the proofs involved a more technical endeavour, but also yields a better understanding of simple tabulation hashing. Later we use this improved understanding of simple tabulation hashing to prove that permutation-tabulation hashing gives Chernoff concentration which up to $O$-notation matches that from the fully random setting even for arbitrary value functions. (This is the content of~\Cref{thm:intro-tab-perm}.)
The hardness of the proof of~\Cref{thm:simpleConcentration} is captured in the case of unit weight balls -- the generalisation to weight functions of bounded support is a mere technicality. Where the paper conceptually breaks new ground in this section is in applying martingale concentration results to obtain a bound on the sum of the squared deviations in the bins which is~\cref{eq:squares} of~\Cref{thm:simpleConcentration}. We proceed to describe this technique starting with a brief description of martingales.
%Where the paper technically breaks new ground in this section is on two counts: the application of martingale concentration bounds and the idea of bounding the sum of the squared deviations of the bins.



%However, we add several further technical contributions towards a much more complete theory of the behaviour of simple tabulation.
%The first obvious difference in this paper, is that we generalize everything to handle arbitrary value functions. This requires careful technical consideration, but does not in and of itself contain any groundbreaking ideas. Where the paper technically breaks new ground in this section is on two counts: the application of martingale concentration bounds and the idea of bounding the sum of the squared deviations of the bins.

Colloquially, a martingale\footnote{A more general and formal definition of a martingale is used in the body of the paper and can be found in the preliminaries.} is a sequence of random variables $X_0, X_1, X_2 \dots$ satisfying that for any $n\in \N$, $\EC{X_{n+1}}{X_0, \dots, X_n}=X_n$. In the modern theory of stochastic processes, martingales are one of the most fundamental objects. A natural way to construct a martingale is through martingale differences. A martingale difference is a sequence of random variables $Y_0, Y_1, \dots$ satisfying that for any $n\in \N$, $\EC{Y_{n+1}}{Y_0, \dots, Y_n}=0$. The name derives from the fact that the sum $X_n = \sum_{i=0}^n Y_i$ is a martingale. A large body of work exists generalizing concentration inequalities for sums of independent random variables to martingales. In this paper, we mainly use a generalization of Bennett's inequality \cite{BennetInequality} by Fan, Grama, and Liu \cite{FanGramaLiu} that allows Chernoff-style bounds for a martingale sequence $X_0, \dots, X_n$ given an almost sure bound for any $i\in [n]$ on the increase of the martingale at step $i$, $\abs{X_i-X_{i-1}}\leq M$ and on the conditional variance $\VarC{X_i}{X_0, \dots, X_{i-1}}\leq \sigma^2$. Now, the applicability to the analysis of simple tabulation is very roughly the following: As discussed above, the analysis proceeds by considering the application of simple tabulation hashing as a process of fixing the hash value of the position characters under $h$ one at a time. Fixing the hash value of  a position character is independent of the previous events so letting $Z_i$ be the value added from the ball in $G_i$ when fixing $h(\alpha_i)$ and $Y_i=Z_i-\E{Z_i}$, $Y_i$ is a martingale difference. Using the inductive hypothesis on the group $G_i$, we obtain the bound $\abs{Y_i}\leq M$ with high probability. Combined with a bound on the variance $\VarC{Y_i}{Y_1, \dots, Y_{i-1}}$ we can apply the martingale concentration inequality described above.

The key to the above strategy being successful is a bound on on the variance of $Y_i$ given $Y_0, \dots, Y_{i-1}$. This is accomplished using another martingale sequence as above. This sequence describes the sum of the squared deviations of each bin from its mean. Informally, this is a martingale of the variance and one would think that the approach runs into the same problem as before, since we now need a bound on the variance of the variance, leading to an endless cycle passing to higher and higher moments. However, it turns out that it is possible to get by with Markov's inequality and a tight, combinatorial analysis of a quantity relating to the number of collisions between sets of keys. %as specified by the following lemma.\todo{Make sure lemma matches}
%\begin{replemma}{lem:CollBound}
%            Let $\ell$ be even and sets of keys $A_1, \dots, A_\ell\subset \Sigma^c$ be given and for each $x\in \Sigma^c$ let $w_x\in [0, 1]$ be some value. Then
      %      \begin{align*}
%                \sum_{\substack{(x_1, \ldots, x_\ell)\in A_1\times \ldots \times A_\ell\\ \bigoplus_{k=1}^\ell x_k = \emptyset}} \prod_{k=1}^\ell w_{x_k}\leq ((\ell-1)!!)^c\cdot \prod_{k=1}^\ell \left(\sqrt{\sum_{x\in A_k}w_x^2}\right).
%            \end{align*}
%\end{replemma}
%In fact this is a generalization of a lemma from~\cite{DKRT15:k-part} which gives the result in case all balls are of unit weight. \todo{I think we have to mention this but it diminishes the novelty...}
Armed with this, we get a bound on the expectation of higher moment bounds, which leads to a bound on the conditional variance of the square deviations of the bins. It thus becomes possible to prove~\cref{eq:squares} of~\Cref{thm:simpleConcentration}.
% \todo{Make sure theorem matches}
% \begin{reptheorem}{thm:sum-squares}
% Let $h\colon \Sigma^c \to [m]$ be a simple tabulation hash function and
 %   $S\subset \Sigma^c$ be a set of keys. Let $w\colon \Sigma^c \times [m] \to [-1, 1]$
 %   a value function satisfying that
  %  $Q = \setbuilder{i \in [m]}{\exists x \in \Sigma^c : w(x, i) \neq 0}$, $\abs{Q} \le m^{\eps}$,
  %  where $\eps < \frac{1}{4}$ is a constant.
  %  Define the random variable
  %  \[
  %      W = \sum_{j \in [m]}\left( \sum_{x \in S}\sum_{k \in Q}
  %          w(x, k)\left([h(x) = j \oplus k] -\frac{1}{m}\right)
  %      \right)^2 \; .
  %  \]
  %    For any $\gamma \geq 1$:
  %  \[
      %  \PR{W \ge (C\gamma)^c\left(\sum_{x \in S}\sum_{k \in Q} w(x, k)^2 \right)}
       %     \le O_{\gamma, \eps, c}\left(\abs{S} m^{-\gamma}\right) \; ,
   % \]
    %where $C = \sqrt{3} \cdot 8$.
 %\end{reptheorem}
Having established this result we apply it to obtain~\cref{eq:Chernoff} of~\Cref{thm:simpleConcentration}.


\subsection{Permutation Yields General Value Functions}
Suppose that we have a hash function $h\colon [u]\to[m]$ satisfying that for any value function $w\colon [u]\times [m] \to [-1, 1]$ supported on $\leq m^\eps$ bins for some $\eps \ge \Omega(1)$, (that is, satisfying that $w(x,i)\neq 0$ only for $i\in Q$ for some set $Q$ of size at most $m^{\eps}$,) we have Chernoff-style bounds on the distribution of the sum $\sum_{x\in [u]}w(x, h(x))$. Furthermore, we have a technical requirement on a squared sum of deviations relating to $h$. This is exactly what we show regarding simple tabulation hashing. To lift the requirement on the support, we propose the following solution. Pick a uniformly random permutation $\tau\colon [m]\times [m]$. We then prove (\Cref{thm:valuefunctions}) that the composition $\tau\circ h$ will have Chernoff-style bounds on the distribution of $V=\sum_{x\in [u]}w(x, \tau\circ h(x))$ for any weight function $w\colon [u]\times [m]\to [-1, 1]$. We loosely sketch this proof in the following. The full proof along with the statement of the theorem can be found in~\Cref{sec:valuefunctions}.

We can suppose up to loss of constant factors that for every $i\in [m]$, $\sum_{x\in [u]}w(x, i)=0$. Denote by $\sigma_i^2=\sum_{x\in [u]}w(x, i)^2$, the ``variational contribution'' of bin $i$. In the fully random setting, the variance $\sigma^2=\Var V$ is $\sigma^2=\sum_{i\in [m]}\sigma_i^2$.
So long as no $\sigma_i^2$ is large, e.g.\ $\sigma_i^2<\sigma^2/m^\eps$ for every $i\in [m]$, we show that the distribution of $V$ obeys Chernoff-style bounds. This allows us to complete the proof in two steps.

First, we consider the $m^\eps$ bins with the largest contributions to the variance. Denote this set of bins by $S\subset[m]$. Fixing the permutation $\tau$ and defining a new value function $w_1\colon [u]\times [m]\to [-1, 1]$ by
\begin{align*}
     w_1(x, i) = \begin{cases}
                            w(x, \tau^{-1}(i)), & i\in S\\
                            0, & i\not\in S.
                        \end{cases}
\end{align*}
Now, this weight function has support on $m^\eps$ bins, so we can apply the assumption on $h$ to get Chernoff-style bounds on the sum $\sum_{x\in S}w(x, \tau\circ h(x))=\sum_{x\in [u]}w_1(x, h(x))$.

Second, by choice of $S$, the remaining bins all have small variance, i.e.\ $\sigma_i^2\leq \sigma^2/m^\epsilon$ for every $i\in [m]\setminus S$. Thus, applying the lemma mentioned above to the value function $w_2\colon [u]\times[m]\to [-1, 1]$ given by
\begin{align*}
    w_2(x, i) = \begin{cases}
                w(x, i), & i\in S,\\
                0, & i\not\in S,
    \end{cases}
\end{align*}
we get Chernoff-style bounds on the sum $\sum_{x\in [u]\setminus S}w(x, \tau\circ h(x)) = \sum_{x\in [u]}w_2(x, \tau\circ h(x))$.

Combining the two observations above yields Chernoff-style bounds on the entire sum $V=\sum_{x\in [u]}w(x, \tau\circ h(x))$ as desired.









\subsection{Extending the Codomain}
The conclusion of the first two parts of the paper is that for universe $[u]=\Sigma^c$, composing a simple tabulation hash function $h\colon \Sigma^c\to [m]$ with a uniformly random permutation $\tau\in S_m$ yields a hash function $g=\tau\circ h$ that for every value function $w\colon \Sigma^c\times [m]\to [0, 1]$ has Chernoff-style concentration bounds on the sum $\sum_{x\in [u]} w(x, g(x))$. This construction works well when $m$ is small, e.g.\ $m\leq \abs\Sigma$. However, since the table required to store $\tau$ has size $\Theta(m)$, it is infeasible for large $m$. For instance, if $m=u$ we might as well have stored a fully random hash function from $[u]$ to $[m]$.

Consequently, we formulate and prove a general theorem capable of extending the codomain of any hash function supporting Chernoff-style bounds on general value functions. We restate the theorem informally for intuition.

Suppose that $a\colon [u]\to B_a$ and $b\colon [u]\to B_b$, respectively, are independently distributed hash functions satisfying that for every choice of weight functions $w_a\colon [u]\times A\to [0, 1]$ and $w_b\colon [u]\times B\to [0, 1]$, the sums $\sum_{x\in [u]}w_a(x, a(x))$ and $\sum_{x\in [u]}w_b(x, b(x))$ are each distributed such that they obey Chernoff-style bounds up to constant factors.
The hash function $c\colon [u]\to B_a\times B_b$ given by $c(x) = (a(x), b(x))$ then satisfies, up to constant factors, Chernoff-style bounds on the distribution of the sum $\sum_{x\in [u]}w_c(x, c(x))$ for every weight function $w_c\colon [u]\times (B_a\times B_b)\to [0, 1]$.

The proof of this theorem crucially relies on the fact that any weight function $w_a$ or $w_b$ can be chosen. Writing $c=(c_1, c_2)$, the key trick is to choose $w_a(x, y) = \EC{w_c(x, c(x))}{c_1(x) = y}$. In this way the analysis can be divided in two. First, one proves that conditioning on the choice of $a$, the mean value stays within an appropriate range with high probability. We also bound the number of keys that become very ``heavy'' after the conditioning. This is done using the assumption on $a$. Second, we use the assumption on $b$ to show that applying $b$ to the value functions arising from conditioning on $a$, we get Chernoff-style probability bounds and lose only constant multiplicative factors.



\subsection{On the Addition of a Query Ball}
Recall that the theorems stated above each contained the condition that they would still hold when the value functions depended on the hash value of some query key $q$. Call this condition $Q$. Reading the body of the paper, one will notice that there is no mention of condition $Q$. This is for two reasons. First, the exposition is already notationally and conceptually heavy without the condition, so excluding the condition enhances readability of the paper. Second, the addition of condition $Q$ adds very little conceptual difficulty. Hence, we have elected instead to sketch the arguments necessary for the addition in a section at the end of the paper.

